DECAF: Deep Extreme Classification with Label Features

Extreme multi-label classification (XML) involves tagging a data point with its most relevant subset of labels from an extremely large label set, with several applications such as product-to-product recommendation with millions of products. Although leading XML algorithms scale to millions of labels, they largely ignore label meta-data such as textual descriptions of the labels. On the other hand, classical techniques that can utilize label metadata via representation learning using deep networks struggle in extreme settings. This paper develops the DECAF algorithm that addresses these challenges by learning models enriched by label metadata that jointly learn model parameters and feature representations using deep networks and offer accurate classification at the scale of millions of labels. DECAF makes specific contributions to model architecture design, initialization, and training, enabling it to offer up to 2-6% more accurate prediction than leading extreme classifiers on publicly available benchmark product-to-product recommendation datasets, such as LF-AmazonTitles-1.3M. At the same time, DECAF was found to be up to 22x faster at inference than leading deep extreme classifiers, which makes it suitable for real-time applications that require predictions within a few milliseconds. The code for DECAF is available at the following URL https://github.com/Extreme-classification/DECAF.

==> sections/ablations.tex <==
\section{Ablation experiments}
\label{sec:ablation}

This section includes ablation experiments to further understand the utility of \alg's components, {\it i.e.,} initialization strategy, label metadata, and classifier. The results are also included for the existing classifiers with explicit label metadata components.

\subsection{Metadata in existing XML algorithms}
\textbf{Learning metadata with base XML classifier}: In principle, \alg's formulation could be efficiently deployed with existing algorithms where collaborative learning among labels is possible. Incorporating label metadata component lead to $1.5\%$ gain in the leading classifier including DiSMEC, Parabel, Bonsai, and DeepXML as compared to their counterparts without the label metadata component. For details please refer to table~\ref{tab:bowmeta} in the supplementary. This demonstrates that label metadata can lead to gains even for current XML algorithms. However, \alg could be upto $3\%$ more accurate as compared to these algorithms even after incorporating label metadata. This demonstrates the utility of \alg's formulation, which efficiently encodes label metadata and encourages collaborative learning among the labels.

\textbf{Re-ranking labels based on label meta-data}:
Classifiers such as DeepXML~\citep{dahiya2020} utilized a re-ranker to improve classification accuracy. \alg's metadata enriched classifier can also be used to re-rank the base classifier's predictions. The re-ranker is the same as the \alg classifier for the leaf nodes (Section~\ref{sec:training}) on the PLT with a difference that top $r$ shortlist of labels are sampled from the base model. In particular, re-ranking Parabel's and DeepXML's predictions could lead to 2\% and 1\% gains compared to the respective base classifiers. However, \alg's label metadata enriched PLT classifier could be upto 4\% more accurate than existing leading XML classifiers, even if they include metadata re-ranker, indicating efficiency as well as the accuracy of the proposed PLT. Please refer to table~\ref{tab:sub:xmlclass} and section~\ref{sup:xmlmeta} in supplementary for more details. 

\subsection{Varying \alg's classifier}
Experiments were also performed to understand the importance of both components of the classifier, \ie, the traditional weight-vector $\v u$, labels metadata weight-vector $\v v$, and the initialization of $\v u$. \alg computes $\v w$ as $\v w=\mathbf{f}(\v u, \v v)$, where $\mathbf{f}(.)$ can be non-linear or a linear operator. Please refer to Table~\ref{tab:combouv} in the supplementary material for different variation of $\mathbf{f}(.)$. First, \alg lead to 1\% gains as compared to the variation where $\v u$ was initialized randomly~\citep{glorot10} while other components were kept same as \alg. Please note that even without initialization \alg can be upto $3\%$ more accurate than state-of-the-art XML classifiers. This indicates metadata $\v v$ is essential to improve accuracy over current XML classifiers. Furthermore, configuration $\v w = \v u$, $\v w = \v u$-no-init, refers to case when metadata component $\v v$ is absent like all XML classifiers. It can be observed that $\v w = \v u$ can be upto $3\%$ more accurate than existing XML classifiers while $\v w = \v u$-no-init performs worse than DeepXML. This indicates the importance of initialization for the traditional classifier $\v u$. \alg's current formulation, {\it i.e.,} $\v w = \sigma(\v \alpha) \odot \v u + \sigma(\v \beta) \odot \v v$ could be upto $2\%$ more accurate as compared to simple sum \ie, $\v w = \v u + \v v$. Indicating current, non-linear combination is essential for better accuracy. Figure~\ref{fig:sub:init} in the supplementary divided labels into five equal size bins of increasing frequency. It can be observed from figure~\ref{fig:sub:init} that the accuracy of labels in the bins having low frequency labels increases significantly when metadata $\v v$ is collaboratively learned along with $\v u$. This supports that collaborative learning can lead to significant gains for data improvised labels.

\subsection{Varying \alg's tree configuration}
Experiments were also performed to understand the impact of \alg's tree hyper-parameters, including depth ($D$) and width ($\max(\v B)$) of the tree, where $\v B$ is the set containing the number of nodes at each depth. Shallow and wide trees were empirically observed to be up to $4\%$ more accurate as compared to slim and deep trees. This can be attributed to the fact that the errors made by nodes at shallow depths can prove to be more costly than errors made by nodes near full depth due to the cascading effect of errors in tree-based settings. Furthermore,~\citep{grave17} demonstrated that shallow and wide trees could be more suitable for GPU based implementation. Different tree configurations are included in Table~\ref{tab:sub:tree_sctruc} in the supplementary material. Furthermore, increasing the number of learners could lead to up to $1.7\%$ increase in accuracy. The accuracy plateaued at three learners (or trees), as demonstrated in Figure~\ref{fig:numlearner} in the supplementary material. It should be reiterated that \alg was observed to be an order of magnitude faster at prediction, even with multiple learners relative to leading XML algorithms.


==> sections/dataset_results.tex <==
\section{Results}
\label{sec:results}

\input{tables/results_main_filtered}
\textbf{Datasets and features}: Experiments were conducted on the following four benchmark datasets available at The Extreme Classification Repository~\cite{XMLRepo}: AmazonTitles-300K, AmazonTitles-2M, WikiSeeAlsoTitles-350K, and WikiTitles-500K. It should be noted that AmazonTitles-300K and AmazonTitles-2M are a subset of standard AmazonTitles-670K and AmazonTitles-3M, respectively, created by restricting the label set to the labels for which meta-data was available. Please refer to Table~\ref{tab:stats} for dataset statistics and data processing scripts in the supplementary material.

\textbf{Evaluation}: Performance was evaluated using popular extreme classification metrics~\cite{Babbar19, Prabhu14, Prabhu18b, dahiya2020, You18, Liu17}, {\it i.e.,} Precision ($P@k$), nDCG ($N@k$) for $k= 1, 3, 5$. These metrics are defined in section~\ref{sup:eval} in the supplementary material. Furthermore, it was observed that documents were mapped to itself in some of the datasets. For instance, `Dinosaur' was tagged with `Dinosaur' label in the AmazonTitles-300K dataset. An algorithm can achieve disproportionately high precision@$1$ by just predicting such labels {\it a.k.a.} trivial predictions, without learning anything useful. Furthermore, such predictions do not add any utility to the quality of predictions in real-life applications. Hence, methods were not rewarded for trivial predictions. Table~\ref{tab:baelines_eval} reports numbers as per this evaluation strategy. All training times have been reported on a 6-core Intel Skylake 2.4 GHz machine with a single Nvidia V100 GPU.

\textbf{Baseline algorithms}: \alg was compared to deep extreme classifiers including XT~\cite{Wydmuch18}, DeepXML~\cite{dahiya2020}, AttentionXML~\cite{You18}, and MACH~\cite{Medini2019}. Furthermore, \alg was also compared to standard extreme classifiers based on sparse BoW features including Bonsai~\cite{Khandagale19}, DiSMEC~\cite{Babbar17}, Parabel~\cite{Prabhu18b}, AnnexML~\cite{Tagami17} and Slice~\cite{Jain19}. Note that Slice was trained with FastText~\cite{Bojanowski16} features while other methods used sparse BoW features. \alg was also compared to a Siamese network learned using triplet loss to embed similar items together. Unfortunately, X-Bert~\citep{Chang19} and GLaS~\citep{Guo2019} could not be included in the analysis as their code was not publicly available.

\textbf{Results on publicly available datasets}: Table~\ref{tab:baelines_eval} compares \alg with leading XML algorithms. Parabel~\citep{Prabhu18}, Bonsai~\citep{Khandagale19}, and AttentionXML~\citep{You18} are the most relevant methods to \alg as they generate a shortlist of negatives based on tree learned in label centroid space. \alg was found to be $5\%$ more accurate than Parabel, Bonsai, and AttentionXML. This indicates that metadata based probabilistic label trees can lead to significant accuracy gains as compared to the counterparts which do not utilize the label meta-data. \alg was also compared with other deep learning based approaches like DeepXML~\cite{dahiya2020}, MACH~\citep{Medini2019}, and XT~\cite{Wydmuch18}. \alg could be upto $4\%$ more accurate while being upto $10\times$ faster at prediction as compared to deep extreme classifiers on a single GPU. Siamese networks included in this analysis had access to the same label metadata information as \alg. However, \alg could be up to $12-18\%$ more accurate than a Siamese network at an extreme scale. Finally, \alg was also compared against other XML classifiers including Slice~\cite{Jain19}, PfastreXML~\cite{Jain17}, DiSMEC~\cite{Babbar17}, AnnexML~\cite{Tagami17}. \alg lead to $4-10\%$ more accurate predictions as compared to these algorithms. This demonstrates that learning tasks-specific features can lead to significantly more accurate predictions. It should be re-iterated that the focus of the paper is short-text documents. Nevertheless, the results on standard full-text versions of the datasets are included in Table~\ref{tab:sup:fulltext} in the supplementary material for the sake of completeness.

\textbf{Analysis}:
\alg encourages collaborative learning among labels which results in more accurate classifiers. Table~\ref{tab:examples} in the supplementary material include examples which demonstrate that \alg was able to predict labels such as ``DC connector", ``RCA connector," and ``Optical fiber connector" when other methods failed to do so. Note that these labels do not share any common training instance but are semantically similar. To better understand the nature of \alg's gains, the label set is divided into five uniform bins~(quantiles) based on the frequency of labels occurring in the training set. While \alg lead to gains in every quantile, the gains were more prominent on data-scarce labels, as demonstrated in Figure~\ref{fig:sup:contrib} in the supplementary material. In conclusion, data improvised tail labels are benefited from collaborative learning and give significant gains in overall accuracy.

==> tables/ablation_tree_structure.tex <==
\begin{table*}
\caption{Effect of varying depth and width of the tree on performance of \alg for AmazonTitles-300K dataset. Empirically, shallow and wider trees were observed to be more accurate than deep trees. Here, $D$ and $\v B$ are the depth and width of the tree, respectively.}
    \label{tab:sub:tree_sctruc}
    \centering
    \begin{tabular}{@{}l|l|cc|cc@{}}
    \toprule
    \textbf{Variation} & \textbf{Configuration} &\textbf{P@1} & \textbf{P@5} & \textbf{PSP@1} & \textbf{PSP@5} \\
    \midrule
\multirow{3}{*}{Width}& $D$=1, $\log(\v B^{k})$=17|19	(\alg) & \textbf{37.88}	 & \textbf{21.09}	 & \textbf{29.68}	 & \textbf{36.76}	 \\
& $D$=1, $\log(\v B^{k})$=15|19	 & 35.55	 & 20.14	 & 26.75	 & 34.35	 \\
& $D$=1, $\log(\v B^{k})$=13|19	 & 33.04	 & 18.19	 & 24.25	 & 30.42	 \\
\midrule
\multirow{3}{*}{Depth}& $D$=1 $\log(\v B^{k})$=17|19	(\alg) & \textbf{37.88}	 & \textbf{21.09}	 & \textbf{29.68}	 & \textbf{36.76}	 \\
& $D$=2, $\log(\v B^{k})$=15|17|19	 & 36.57	 & 20.62	 & 28.01	 & 35.5	 \\
& $D$=3, $\log(\v B^{k})$=13|15|17|19	 & 35.41	 & 19.82	 & 26.73	 & 33.78	 \\
    \bottomrule
    \end{tabular}
\end{table*}

==> tables/notations.tex <==
\begin{table*}[ht]
    \caption{List of notations used in this paper.}
    \label{tab:notations}
    \centering
    \begin{tabular}{c|p{0.75\textwidth}}
        \toprule
        \textbf{Symbol} & \textbf{Meaning} \\
        \midrule
        \multicolumn{2}{c}{Dataset symbols} \\
        \midrule
         $N$ &  Number of documents\\
         $\v L$ & Set containing label indices \\
         $L$ & Size of label set $L = |\v L|$ \\
         $\v x_i$ & TF-IDF valued bag of words representation for document $i$\\
         $\v f_l$ & TF-IDF valued bag of words representation for label $l$\\
         $\v y_i$ & Ground truth for document $i$\\
        \midrule
        \multicolumn{2}{c}{Tree symbols} \\
        \midrule
         $D$ & Depth of tree \\
         $\v B$ & Set containing number of nodes at each depth \\
         $\Lf{n}{k}$ & Set of labels at the leaf nodes of sub tree rooted at node $n$ of depth $k$ \\
         $\pt{l}{k}$ & Index of node at depth $k$ such that $l \in \Lf{\pt{l}{k}}{k}$\\
         \multirow{3}{*}{$r$} & Beam size used for selecting most probable nodes at each depth of the tree. Please note that we can have different $\rp{k}$ for each depth $k$. However, for the simplicity we have used same $r$. \\
        \midrule
        \multicolumn{2}{c}{Model symbols} \\
        \midrule
         $\mathcal{LL}$ & Exact log likelihood used by \alg \\
         $\mathcal{LL}^{'}$ & Approximation of $\mathcal{LL}$ for scalable training \\
         $\v E_x^{k} $ & Shared Token embedding for documents at depth $k$ \\
         $\v E_y^{k} $ & Shared Token embedding for label titles at depth $k$ \\
         $\v z^{k}$ & Document representation at depth $k$ \\
         $\v u^{k}_{j}$ & Traditional classifier initialized with label metadata for node $j$ at depth $k$\\
         $\v v^{k}_{j}$ & Classifier generated from label metadata for node $j$ at depth $k$ \\
         $\v \alpha^{k}$ & Weightage of $\v u^{k}_{j}$ which is learning at the time of training for depth $k$ \\
         $\v \beta^{k}$ & Weightage of $\v v_{j}^{k}$ which is learning at the time of training for depth $k$ \\
         \bottomrule
         
    \end{tabular}
\end{table*}

==> tables/results_main_filtered.tex <==
\begin{table*}[ht]
    \caption{\alg was found to be 4--10\% more accurate on the standard benchmark datasets. Additionally, it could be an order of magnitude faster in prediction as compared to deep learning based approaches. Algorithms marked with `-' were unable to scale on given dataset in the available resources.}
    \label{tab:baelines_eval}
    \begin{subtable}{.48\textwidth}
      \centering
      \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}l|ccc|c@{}}
        \toprule
        \textbf{Method} & \textbf{P@1} & \textbf{P@3} & \textbf{P@5} &  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Prediction}\\ \textbf{Time (ms)}\end{tabular}} \\
        \midrule
            \multicolumn{5}{c}{AmazonTitles-300K}\\
        \midrule
        \midrule
\alg	 & \textbf{37.88}	 & \textbf{27.78}	 & \textbf{21.09}	 & \textbf{0.11} \\
AttentionXML	 & 26.87	 & 19.82	 & 15.01	 & 11.7 \\
Bonsai	 & 32.88	 & 24.69	 & 18.79	 & 9.06 \\
Parabel	 & 31.77	 & 23.75	 & 17.99	 & 1.05 \\
AnneXML	 & 27.96	 & 21.85	 & 17.4	 & 1.14 \\
XT	 & 30.7	 & 23.46	 & 18.08	 & 4.73 \\
DeepXML	 & 34.54	 & 25.97	 & 19.8	 & 2.17 \\
MACH	 & 31.68	 & 24.02	 & 18.38	 & 1.18 \\
Slice	 & 30.96	 & 23.36	 & 17.91	 & 1.46 \\
DiSMEC	 & 32.77	 & 25.01	 & 19.18	 & 6.25 \\
PfastreXML	 & 30.54	 & 23.28	 & 17.96	 & 4.35 \\
Siamese	 & 20.29	 & 13.1	 & 9.66	 & 9.74 \\
\midrule \multicolumn{5}{c}{AmazonTitles-2M}\\ \midrule \midrule				
\alg	 & \textbf{64.02}	 & \textbf{59.55}	 & \textbf{56.33}	 & \textbf{0.13} \\
AttentionXML	 & -	 & -	 & -	 & - \\
Bonsai	 & 61.57	 & 57.22	 & 54.05	 & 45.03 \\
Parabel	 & 60.55	 & 56.38	 & 53.32	 & 0.85 \\
AnneXML	 & 59.69	 & 55.79	 & 53	 & 1.46 \\
XT	 & 38.13	 & 34.91	 & 32.73	 & 3.78 \\
DeepXML	 & 58.51	 & 54.27	 & 51.19	 & 3 \\
MACH	 & -	 & -	 & -	 & - \\
Slice	 & 45.76	 & 42.47	 & 40.03	 & 0.83 \\
DiSMEC	 & -	 & -	 & -	 & - \\
PfastreXML	 & 48.96	 & 47.25	 & 45.66	 & 19.48
\\
\bottomrule
        \end{tabular}}
    \end{subtable}
    ~
    \begin{subtable}{.48\textwidth}
      \centering
      \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}l|ccc|c@{}}
        \toprule
        \textbf{Method} & \textbf{P@1} & \textbf{P@3} & \textbf{P@5} &  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Prediction}\\ \textbf{Time (ms)}\end{tabular}} \\
        \midrule \multicolumn{5}{c}{WikiSeeAlsoTitles-350K} \\ \midrule
        \midrule
\alg	 & \textbf{27.56}	 & \textbf{19.68}	 & \textbf{15.35}	 & \textbf{0.11} \\
AttentionXML	 & 15.61	 & 9.83	 & 7.36	 & 8.79 \\
Bonsai	 & 20.73	 & 14.42	 & 11.13	 & 12.6 \\
Parabel	 & 19.52	 & 13.33	 & 10.24	 & 1.02 \\
AnneXML	 & 16.34	 & 11.55	 & 9.21	 & 1.24 \\
XT	 & 18.73	 & 13.08	 & 10.23	 & 4.26 \\
DeepXML	 & 23.89	 & 16.78	 & 13	 & 2 \\
MACH	 & 16.62	 & 10.98	 & 8.24	 & 1.98 \\
Slice	 & 21.23	 & 15.28	 & 12.14	 & 1.27 \\
DiSMEC	 & 17.67	 & 12.01	 & 9.35	 & 9.07 \\
PfastreXML	 & 17.88	 & 12.43	 & 9.58	 & 3.59 \\
Siamese	 & 14.03	 & 8.95	 & 6.72	 & 10.69 \\
\midrule \multicolumn{5}{c}{WikiTitles-500K}\\ \midrule \midrule				
\alg	 & \textbf{47.72}	 & \textbf{27.12}	 & \textbf{19.33}	 & \textbf{0.11} \\
AttentionXML	 & 42.59	 & 22.39	 & 15.61	 & 8.79 \\
Bonsai	 & 42.58	 & 23.06	 & 16.22	 & 16.09 \\
Parabel	 & 42.45	 & 23.01	 & 16.17	 & 1.02 \\
AnneXML	 & 39.47	 & 20.52	 & 14.33	 & 1.24 \\
XT	 & 40.09	 & 21.99	 & 15.6	 & 4.26 \\
DeepXML	 & 45.3	 & 25	 & 17.7	 & 2.71 \\
MACH	 & 33.68	 & 15.64	 & 10.43	 & 1.98 \\
Slice	 & 28.17	 & 16.85	 & 12.34	 & 1.06 \\
DiSMEC	 & 39.89	 & 21.23	 & 14.96	 & 9.07 \\
PfastreXML	 & 30.97	 & 18.1	 & 13.12	 & 7.79 \\
\bottomrule
        \end{tabular}}
    \end{subtable} 
\end{table*}

==> tables/results_sup_filtered_ndcg.tex <==
\begin{table}[ht]
\caption{\alg is more accurate on all evaluation metrics, and a order of magnitude faster in prediction as compared to deep learning based approaches.}
    \label{tab:baelines_eval_ndcg}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}c|l|cc|cc@{}}
    \toprule
    \textbf{Dataset} & \textbf{Method} & \textbf{N@1} & \textbf{N@5} & \textbf{PSN@1} & \textbf{PSN@5} \\
    \midrule
     \multirow{13}{*}{\textbf{\rotatebox{90}{AmazonTitles-300K}}}	 & \algp	 & \textbf{38.18}	 & \textbf{21.21}	 & \textbf{30.01}	 & \textbf{36.89} \\
	 & Co-XML	 & 37.06	 & 20.71	 & 28.5	 & 35.55 \\
	 & DeepXML	 & 34.54	 & 19.8	 & 26.12	 & 33.85 \\
	 & AttentionXML	 & 26.87	 & 15.01	 & 18.61	 & 24.03 \\
	 & XT	 & 30.7	 & 18.08	 & 21.47	 & 29.71 \\
	 & MACH	 & 31.68	 & 18.38	 & 22.3	 & 30.3 \\
	 & KNN-Fasttext	 & 23.65	 & 11.82	 & 23.36	 & 24.11 \\
	 & KNN-Bert	 & 18.86	 & 8.89	 & 18.53	 & 17.88 \\
	 & Siamese	 & 20.29	 & 9.66	 & 19.68	 & 19.54 \\
	 & Slice	 & 30.96	 & 17.91	 & 22.99	 & 30.62 \\
	 & Parabel	 & 31.77	 & 17.99	 & 22.3	 & 29.59 \\
	 & DiSMEC	 & 32.77	 & 19.18	 & 23.23	 & 32.26 \\
	 & AnneXML	 & 27.96	 & 17.4	 & 17.03	 & 27.3 \\
	 \midrule
	 \multirow{13}{*}{\textbf{\rotatebox{90}{WikiSeeAlsoTitles-350K}}}	 & \algp	 & \textbf{27.95}	 & \textbf{15.33}	 & \textbf{16.99}	 & \textbf{21.44} \\
	 & Co-XML	 & 27.24	 & 14.78	 & 16.04	 & 20.17 \\
	 & DeepXML	 & 23.89	 & 13	 & 13.29	 & 17.61 \\
	 & AttentionXML	 & 15.61	 & 7.36	 & 6.67	 & 7.58 \\
	 & XT	 & 18.73	 & 10.23	 & 9.36	 & 12.57 \\
	 & MACH	 & 16.62	 & 8.24	 & 7.96	 & 9.54 \\
	 & KNN-Fasttext	 & 16.41	 & 8.82	 & 14.71	 & 16.3 \\
	 & KNN-Bert	 & 11.12	 & 5.74	 & 10.27	 & 10.86 \\
	 & Siamese	 & 14.03	 & 6.72	 & 12.52	 & 12.55 \\
	 & Slice	 & 21.23	 & 12.14	 & 11.4	 & 16.26 \\
	 & Parabel	 & 19.52	 & 10.24	 & 9.63	 & 12.51 \\
	 & DiSMEC	 & 17.67	 & 9.35	 & 8.54	 & 11.31 \\
	 & AnneXML	 & 16.34	 & 9.21	 & 6.78	 & 10.6 \\
	 \midrule
	 \multirow{13}{*}{\textbf{\rotatebox{90}{WikiTitles-500K}}}	 & \algp	 & \textbf{47.34}	 & \textbf{18.54}	 & 19.79	 & \textbf{19.93} \\
	 & Co-XML	 & 47.24	 & 18.49	 & \textbf{19.89}	 & 19.77 \\
	 & DeepXML	 & 45.3	 & 17.7	 & 18.45	 & 18.41 \\
	 & AttentionXML	 & 42.59	 & 15.61	 & 14.98	 & 13.9 \\
	 & XT	 & 40.09	 & 15.6	 & 15.44	 & 15.57 \\
	 & MACH	 & 33.68	 & 10.43	 & 11.37	 & 8.37 \\
	 & KNN-Fasttext	 & 16.71	 & 5.59	 & 16.36	 & 11.03 \\
	 & KNN-Bert	 & 8.33	 & 2.7	 & 8.61	 & 5.61 \\
	 & Siamese	 & -	 & -	 & -	 & - \\
	 & Slice	 & 28.17	 & 12.34	 & 15.17	 & 15.41 \\
	 & Parabel	 & 42.45	 & 16.17	 & 16.5	 & 16.12 \\
	 & DiSMEC	 & 39.89	 & 14.96	 & 15.97	 & 15.46 \\
	 & AnneXML	 & 39.47	 & 14.33	 & 13.92	 & 13.29 \\
	 \midrule
	 \multirow{10}{*}{\textbf{\rotatebox{90}{AmazonTitles-1.6M}}}	 & \algp	 & \textbf{48.1}	 & \textbf{42.99}	 & 14.45	 & 18.91 \\
	 & Co-XML	 & 45.53	 & 40.5	 & 14.4	 & 18.45 \\
	 & DeepXML	 & 45.46	 & 41.37	 & \textbf{16.44}	 & \textbf{20.55} \\
	 & AttentionXML	 & -	 & -	 & -	 & - \\
	 & XT	 & -	 & -	 & -	 & - \\
	 & MACH	 & -	 & -	 & -	 & - \\
	 & Slice	 & 35.29	 & 31.7	 & 11.48	 & 15.19 \\
	 & Parabel	 & 46.52	 & 41.73	 & 13.11	 & 17.72 \\
	 & DiSMEC	 & -	 & -	 & -	 & - \\
	 & AnneXML	 & 47.43	 & 42.14	 & 11.63	 & 16.47 \\
    \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/results_sup_unfiltered.tex <==
\begin{table}[h]
\caption{\alg is more accurate on all evaluation metrics, and a order of magnitude faster in prediction as compared to deep learning based approaches.}
    \label{tab:sup:baelines_eval_unfilters}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}c|l|ccccc|ccccc@{}}
    \toprule
    \textbf{Dataset} & \textbf{Method} & \textbf{P@1=N@1} & \textbf{P@3} & \textbf{P@5} & \textbf{N@3} & \textbf{N@5} & \textbf{PSP@1}=\textbf{PSN@1} & \textbf{PSP@5} & \textbf{PSN@5} \\
    \midrule
  \multirow{10}{*}{\textbf{\rotatebox{90}{AmazonTitles-300K}}}	 & \alg(T=3)	 & \textbf{58.39}	 & \textbf{30.19}	 & \textbf{49.71}	 & \textbf{48.31}	 & \textbf{45.15}	 & \textbf{45.62} \\
	 & \alg -uni (T=3)	 & 57.02	 & 29.48	 & 48.53	 & 46.68	 & 43.69	 & 44.1 \\
	 & DeepXML	 & 36.01	 & 23.03	 & 35.16	 & 26.45	 & 32.65	 & 29.77 \\
	 & AttentionXML	 & 28.38	 & 17.27	 & 26.21	 & 18.15	 & 22.38	 & 19.89 \\
	 & XT (T=3)	 & 32.6	 & 20.89	 & 31.65	 & 21.05	 & 27.77	 & 24.68 \\
	 & MACH	 & 33.66	 & 21.25	 & 32.54	 & 21.96	 & 28.39	 & 25.64 \\
	 & Slice+Fasttext	 & 33.08	 & 21.17	 & 32.29	 & 22.7	 & 29.36	 & 26.53 \\
	 & ParabelOld	 & 33.72	 & 20.84	 & 31.86	 & 21.84	 & 27.75	 & 24.92 \\
	 & DiSMEC	 & 34.86	 & 22.45	 & 34.29	 & 22.82	 & 30.63	 & 27.53 \\
	 & AnnexML	 & 29.05	 & 19.5	 & 28.78	 & 16.2	 & 24.44	 & 20.64 \\
	 \midrule
	 \multirow{10}{*}{\textbf{\rotatebox{90}{WikiSeeAlsoTitles-350K}}}	 & \alg(T=3)	 & 21.15	 & \textbf{14.66}	 & \textbf{25.58}	 & 11.54	 & \textbf{20.37}	 & \textbf{18.51} \\
	 & \alg -uni (T=3)	 & 21.04	 & 14.16	 & 24.89	 & 11.25	 & 19.18	 & 17.61 \\
	 & DeepXML	 & \textbf{21.97}	 & 12.56	 & 22.53	 & \textbf{12.46}	 & 17.34	 & 16.08 \\
	 & AttentionXML	 & 14.91	 & 7.23	 & 13.68	 & 6.15	 & 7.39	 & 7.1 \\
	 & XT (T=3)	 & 17.85	 & 10.02	 & 18.21	 & 8.69	 & 12.23	 & 11.39 \\
	 & MACH	 & 16.04	 & 8.13	 & 15.69	 & 7.5	 & 9.36	 & 9.37 \\
	 & Slice+Fasttext	 & 20.17	 & 11.83	 & 20.95	 & 10.56	 & 15.75	 & 14.27 \\
	 & ParabelOld	 & 18.61	 & 10.04	 & 18.44	 & 8.93	 & 12.17	 & 11.41 \\
	 & DiSMEC	 & 16.61	 & 9.14	 & 16.72	 & 7.75	 & 10.96	 & 10.24 \\
	 & AnnexML	 & 15.74	 & 8.99	 & 16.04	 & 6.37	 & 10.22	 & 9.07 \\
	 \midrule
	 \multirow{10}{*}{\textbf{\rotatebox{90}{WikiTitles-500K}}}	 & \alg(T=3)	 & \textbf{47.34}	 & \textbf{18.54}	 & \textbf{33.7}	 & 19.79	 & \textbf{19.93}	 & \textbf{23.06} \\
	 & \alg -uni (T=3)	 & 47.24	 & 18.49	 & 33.66	 & \textbf{19.89}	 & 19.77	 & 22.98 \\
	 & DeepXML	 & -	 & -	 & -	 & -	 & -	 & - \\
	 & AttentionXML	 & 42.59	 & 15.61	 & 28.53	 & 14.98	 & 13.9	 & 16.44 \\
	 & XT (T=3)	 & 40.09	 & 15.6	 & 28.17	 & 15.44	 & 15.57	 & 17.92 \\
	 & MACH	 & 33.68	 & 10.43	 & 20.81	 & 11.37	 & 8.37	 & 11.28 \\
	 & Slice+Fasttext	 & 28.17	 & 12.34	 & 22.94	 & 15.17	 & 15.41	 & 17.75 \\
	 & ParabelOld	 & 42.45	 & 16.17	 & 29.4	 & 16.5	 & 16.12	 & 18.72 \\
	 & DiSMEC	 & 39.89	 & 14.96	 & 27.31	 & 15.97	 & 15.46	 & 17.9 \\
	 & AnnexML	 & 39.47	 & 14.33	 & 26.52	 & 13.92	 & 13.29	 & 15.65 \\
	 \midrule
	 \multirow{10}{*}{\textbf{\rotatebox{90}{AmazonTitles-1.6M}}}	 & \alg(T=3)	 & \textbf{48.1}	 & \textbf{42.99}	 & \textbf{44.66}	 & \textbf{13.81}	 & \textbf{18.02}	 & \textbf{16.7} \\
	 & \alg -uni (T=3)	 & 45.53	 & 40.5	 & 42.13	 & 13.76	 & 17.58	 & 16.37 \\
	 & DeepXML	 & -	 & -	 & -	 & -	 & -	 & - \\
	 & AttentionXML	 & -	 & -	 & -	 & -	 & -	 & - \\
	 & XT (T=3)	 & -	 & -	 & -	 & -	 & -	 & - \\
	 & MACH	 & -	 & -	 & -	 & -	 & -	 & - \\
	 & Slice+Fasttext	 & 35.29	 & 31.7	 & 32.9	 & 10.97	 & 14.47	 & 13.38 \\
	 & ParabelOld	 & 46.52	 & 41.73	 & 43.32	 & 12.53	 & 16.88	 & 15.55 \\
	 & DiSMEC	 & -	 & -	 & -	 & -	 & -	 & - \\
	 & AnnexML	 & 47.43	 & 42.14	 & 43.74	 & 11.11	 & 15.69	 & 14.25 \\
    \bottomrule
    \end{tabular}
    }
\end{table}
